Grounded Language Understanding for Manipulation Instructions Using GAN-Based Classification

The target task of this study is grounded language understanding for domestic service robots (DSRs). In particular, we focus on instruction understanding for short sentences where verbs are missing. This task is of critical importance to build communicative DSRs because manipulation is essential for DSRs. Existing instruction understanding methods usually estimate missing information only from non-grounded knowledge; therefore, whether the predicted action is physically executable or not was unclear. In this paper, we present a grounded instruction understanding method to estimate appropriate objects given an instruction and situation. We extend the Generative Adversarial Nets (GAN) and build a GAN-based classifier using latent representations. To quantitatively evaluate the proposed method, we have developed a data set based on the standard data set used for Visual QA. Experimental results have shown that the proposed method gives the better result than baseline methods.

==> Makefile <==
#
# Makefile for tex English
# 英語用 latexとbibtex
#
# v??.?jp Time-stamp: "2017-06-26 12:46:20 sugiura"
# v17.6en Time-stamp: "2017-06-26 12:45:25 sugiura"
# v16.11jp Time-stamp: "2016-11-14 14:34:18 sugiura"
# v15.8 Time-stamp: "2015-08-18 14:48:30 sugiura"
# v1.3 Time-stamp: "2012-12-08 01:31:10 sugiura"
#


.SUFFIXES: .tex .dvi .aux .log .toc .lof .lot .pdf .ps .bbl .bib .blg
.PHONY: clean

# コンパイル対象
MAIN		 = main
TEXFILES	 = $(shell ls *.tex)
BIBFILES	 = $(shell ls *.bib)

# -interaction=nonstopmode: latexをサイレントモードで．
TEXOP		 = pdflatex -interaction=nonstopmode 1>/dev/null
TEXOP_DEBUG	 = pdflatex

# -terse: bibtexをサイレントモードで．
BIBTEX		 = bibtex -terse
PDFVIEWER	 = evince

# make cleanで消す対象
TRUSH		 = $(MAIN).dvi $(MAIN).aux $(MAIN).lof $(MAIN).toc $(MAIN).lot $(MAIN).log $(MAIN).pdf $(MAIN).ps $(MAIN).bbl $(MAIN).blg $(MAIN).out $(MAIN).fls


all: $(MAIN).pdf
pdf: $(MAIN).pdf
bbl: $(MAIN).bbl


$(MAIN).pdf:	 $(BIBFILES) $(TEXFILES)
$(MAIN).bbl:	 $(BIBFILES) $(TEXFILES)
$(MAIN).aux:	 $(MAIN).tex

.tex.pdf:
	$(TEXOP) $*; $(BIBTEX) $*; $(TEXOP) $*; $(TEXOP) $*
	cp -f $(MAIN).pdf ~/

.tex.aux:
	$(TEXOP) $*

# ユーティリティコマンド群
viewpdf: $(MAIN).pdf
	$(PDFVIEWER) $< &

debug:
	$(TEXOP_DEBUG) $(MAIN)

clean:
	rm -f *~ \#* $(TRUSH) $(COVERTRUSH) missfont.log

PWD = $(shell pwd)
DIRNAME = $(shell basename $(PWD))

# ページ指定でpdfをブラウザで開く
# 4ページ目を開く場合はmake page P=4とする
browse: $(MAIN).pdf
	firefox	file://$(PWD)/$(MAIN).pdf#page=$(p)

# カレントディレクトリを圧縮して../に置く
tgz: clean
	tar -C .. -cvzf ../$(DIRNAME).tgz $(DIRNAME)

# Local Variables:
# coding: utf-8
# End:


==> fig/classification/lacgan01.tex <==
% %% LyX 2.0.8.1 created this file.  For more info, see http://www.lyx.org/.
% %% Do not edit unless you really know what you are doing.
% \documentclass{article}
% \usepackage[japanese]{babel}

% \makeatletter

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LyX specific LaTeX commands.
% %% Because html converters don't know tabularnewline
% \providecommand{\tabularnewline}{\\}

% \makeatother

% \begin{document}
\begin{tabular}{|c|c|}
\hline 
 & テストセット精度\tabularnewline
\hline 
\hline 
Baseline (AC-GAN, PA無) & 50.7\%\tabularnewline
\hline 
Baseline (AC-GAN, PA有) & 58.2\%\tabularnewline
\hline 
Extractorのみ & 61.1\%\tabularnewline
\hline 
提案手法 (LAC-GAN) & 67.1\%\tabularnewline
\hline 
\end{tabular}
% \end{document}


==> fig/dataset/dataset02.tex <==
% %% LyX 2.0.8.1 created this file.  For more info, see http://www.lyx.org/.
% %% Do not edit unless you really know what you are doing.
% \documentclass{article}
% \usepackage[japanese]{babel}

% \makeatletter

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LyX specific LaTeX commands.
% %% Because html converters don't know tabularnewline
% \providecommand{\tabularnewline}{\\}

% \makeatother

% \begin{document}
\begin{tabular}{|l|c|}
\hline 
データセットサイズ(E1-O) & 896\tabularnewline
\hline 
状況の言語表現に含まれる語彙数 & 7926\tabularnewline
\hline 
状況の言語表現に含まれる平均単語数 & 305\tabularnewline
\hline 
学習セットサイズ(N, M0, M1, M2) & 539\tabularnewline
\hline 
検証セットサイズ(N, M0, M1, M2) & 67\tabularnewline
\hline 
テストセットサイズ(N, M0, M1, M2) & 67\tabularnewline
\hline 
\end{tabular}
% \end{document}


==> fig/settings/settings01.tex <==
% %% LyX 2.0.8.1 created this file.  For more info, see http://www.lyx.org/.
% %% Do not edit unless you really know what you are doing.
% \documentclass{article}
% \usepackage[japanese]{babel}

% \makeatletter

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LyX specific LaTeX commands.
% %% Because html converters don't know tabularnewline
% \providecommand{\tabularnewline}{\\}

% \makeatother

% \begin{document}
\begin{tabular}{|c|c|}
\hline 
最適化手法 & Adam (学習率0.0005,\tabularnewline
 & $\beta_1=0.5$, $\beta_2=0.999$)\tabularnewline
\hline 
E input & Name (200)+ Situation (200)\tabularnewline
\hline 
Eノード数 & 400(in), 400, 100, 50, 100, 4(out)\tabularnewline
\hline 
Gノード数 & 104(in), 100, 100, 50(out)\tabularnewline
\hline 
Dノード数 & 50(in), 100, 100, 5(out)\tabularnewline
\hline 
バッチサイズ & 50(E), 20(G and D)\tabularnewline
\hline 
$\lambda$ & 0.2\tabularnewline
\hline 
\end{tabular}
% \end{document}

